One-Shot Perfect Secret Key Agreement for Finite Linear Sources

We consider a non-asymptotic (one-shot) version of the multiterminal secret key agreement problem on a finite linear source model. In this model, the observation of each terminal is a linear function of an underlying random vector composed of finitely many i.i.d. uniform random variables. Restricting the public discussion to be a linear function of the terminals' observations, we obtain a characterization of the communication complexity (minimum number of symbols of public discussion) of generating a secret key of maximum length. The minimum discussion is achieved by a non-interactive protocol in which each terminal first does a linear processing of its own private observations, following which the terminals all execute a discussion-optimal communication-for-omniscience protocol. The secret key is finally obtained as a linear function of the vector of all observations.

==> preliminaries.tex <==
% Following from the result of G\'acs and K\"orner in \cite{gacs72}, a secret key rate
% achievable without public discussion is as follows:
% \begin{Proposition}
%   \label{pro:>=JGK}
%   $\CS(0)\geq J_{\op{GK}}(\RZ_V)$ where
%   \begin{align}
%     J_{\op{GK}}(\RZ_V) := \max\Set{ H(\RG) \mid H(\RG|\RZ_i)=0,
%     \forall i\in V}\label{eq:JGK}
%   \end{align}
%   is called the (multivariate) G\'acs--K\"orner common information. 
% \end{Proposition}
% The optimal solution $\RG$ is called the maximum common function,
% since it is a function of each $\RZ_i$, and its entropy is
% maximized. It can be shown that every common function of $\RZ_i$'s is
% a function of $\RG$. Although $\RG$ can be computed systematically
% using the ergodic decomposition in \cite{gacs72}, the computation may take
% exponential time.

% The proof of the achievable result is quite straightforward because,
% without any discussion, users can agree on $\RG^n$ perfectly with no
% error. From $\RG^n$, a secret key of rate $H(\RG)$ can be extracted
% by the usual compression technique. The
% challenge is prove the converse and resolve the following conjecture:
% \begin{Conjecture}
%   \label{conj:CS=JGK}
%   $\CS(0)=J_{\op{GK}}(\RZ_V)$.
% \end{Conjecture}

% To simplify the problem, we further consider the following source models.
% \begin{Definition}[\mbox{\cite{chan10md}}]
%   \label{def:hyp}
%   The source $\RZ_V$ is said to be hypergraphical if, for
%   all $i\in V$, $\RZ_i$ is equivalent to
%   \begin{align}
%     (\RX_e\mid e\in E, i\in `x(e)),
%   \end{align}
%   up to bijections,\footnote{$\RZ'_i$ is said to be a bijection of $\RZ_i$ iff $H(\RZ'_i|\RZ_i)=H(\RZ_i|\RZ_i')=0$.} where $E$ is the edge set and $`x:E\to 2^V`/\Set{`0}$ is called the
%   edge function. The hypergraph $(V,E,`x)$ and the edge (random)
%   variables $\RX_e$'s define the source.
% \end{Definition}
% A simple example of the hypergraphical source is as follows:
% \begin{Example}
%   \label{eg:hyp}
%   Let $\RX_a$, $\RX_b$ and $\RX_c$ be uniformly random and independent
%   bits. With $V:=\Set{1,2}$, define
%   \begin{align*}
%     \RZ_1:= (\RX_a,\RX_b,\RX_c), \quad \RZ_2:=(\RX_b,\RX_c),
%     \,\text{ and }\,\RZ_3:=(\RX_a,\RX_c).
%   \end{align*}
%   This source is hypergraphical with $E=\Set{a,b,c}$,
%   $`x(a)=\Set{1,2}$, $`x(b)=\Set{1,3}$ and $`x(c)=\Set{1,2,3}$.
% \end{Example}

% Another source model we will consider is:
% \begin{Definition}[\mbox{\cite{chan10phd}}]
%   \label{def:fls}
%   The source $\RZ_V$ is said to be a finite linear source if, for all $i\in V$, $\RZ_i$ is equivalent to
%   \begin{align}
%     \RMx \MM_i,\label{eq:fls}
%   \end{align}
%   up to bijections, 
%   where $\RMx$ is a uniformly random vectors with elements taking
%   values from some finite field $\bbF_q$, and $\MM_i$ is a
%   deterministic matrix with elements from $\bbF_q$. 
% \end{Definition}
% The following is an example of a finite linear source that is not hypergraphical.
% \begin{Example}
%   \label{eg:fls}
%   Again with $\RX_a$, $\RX_b$ and $\RX_c$ being uniformly random and
%   independent bits, define $V:=\Set{1,2,3}$,
%   \begin{align*}
%     \RZ_1 := \RX_a,\quad
%     \RZ_2 := \RX_b,\,\text{ and }\,
%     \RZ_3 :=\RX_a\oplus \RX_b,
%   \end{align*}
%   where $\oplus$ is the XOR operation. 
%   This is a finite linear source because, with $\RMx:=\bM \RX_a & \RX_b \eM$,
%   \begin{align*}
%     \RZ_1 =\RMx \bM 1 \\ 0 \eM,\quad 
%     \RZ_2 = \RMx \bM 0 \\ 1 \eM,\quad
%     \RZ_3 = \RMx \bM 1\\ 1\eM, 
%   \end{align*}
%   and $\RMx$ is uniformly distributed over $\bbF_2^2$, where the matrix multiplications are over $\bbF_2$, and $\RMx$ is uniformly over $\bbF_2^2$. Note that $\RZ_i$'s are pairwise independent and so there is no edge variable with strictly positive entropy covering more than one node. There is no edge covering one node either, because each $\RZ_i$ is completely determined by other $\RZ_j$'s. However, $H(\RZ_V)=2>0$, and so it cannot be a hypergraphical source with no edge variable.
% \end{Example}


